Privacy via the Johnson-Lindenstrauss Transform

Suppose that party A collects private information about its users, where each user's data is represented as a bit vector. Suppose that party B has a proprietary data mining algorithm that requires estimating the distance between users, such as clustering or nearest neighbors. We ask if it is possible for party A to publish some information about each user so that B can estimate the distance between users without being able to infer any private bit of a user. Our method involves projecting each user's representation into a random, lower-dimensional space via a sparse Johnson-Lindenstrauss transform and then adding Gaussian noise to each entry of the lower-dimensional representation. We show that the method preserves differential privacy---where the more privacy is desired, the larger the variance of the Gaussian noise. Further, we show how to approximate the true distances between users via only the lower-dimensional, perturbed data. Finally, we consider other perturbation methods such as randomized response and draw comparisons to sketch-based methods. While the goal of releasing user-specific data to third parties is more broad than preserving distances, this work shows that distance computations with privacy is an achievable goal.

==> conclusions.tex <==
\section{Conclusion and Future Work}
We proposed a viable solution to the challenge of publishing user data for enabling computation of distance between users, without revealing the values of user data attributes. The key insight behind our technique is that by projecting users to a lower-dimensional space, we can limit the amount of noise we add to each user's data, while also reaping the benefit of preserving distances. We also compared our proposed solution to other candidate solutions, such as directly adding noise to the pairwise distances or adding noise to each attribute of a user, and showed that our method is preferable for potential applications such as user segmentation and nearest neighbor search.

There is ample opportunity to improve upon our results as the problem of privacy-preserving data sharing with third parties is naturally more complex than sharing in a way that enables distance computations. For example, third parties would benefit from data that enables computation of other data-mining primitives and from ability to operate on dynamically changing data~\cite{continuous}. 


==> discussion.tex <==
\section{Discussion}\label{sec:discussion}
In this section, we describe how user sketches released in a privacy-preserving way can be used by third parties, and conclude by discussing the limitations of sketches and our privacy guarantees.

%While we showed that user-dependent sketches can be published in a
%privacy-preserving way, it is natural to ask if these sketches are of
%any use to an advertiser.  and then discuss ways in which
%an advertiser can utilize these sketches.  We also discuss limitations
%of sketches, how to adapt our method to satisfy a more stringent privacy guarantee, as well as limitations of our privacy guarantee.

\subsection{Applications}
We begin by re-iterating exactly what can be safely published:
\squishlisttwo
\item The $d$ attribute meanings in the original vector space,
assuming the meanings themselves are not sensitive, or the ones that are published via a method similar to the one in~\cite{KKMN09} or \cite{Goetz}.

\item The Johnson-Lindenstrauss projection matrix $P$.

\item For each user $x$, their userID, together with their perturbed sketch $xP+\Delta$. %Hence, our approach works well for the scenarios when a trusted online service provider (e.g., Google, Microsoft, Facebook), who collects and possesses information about their users wants to share this information with third parties.
\squishend

There are several actions that the third party can perform with this
published information, depending on what kind of additional information the
third party possesses about the users and the goal the third party is trying to achieve.

{\bf Segmentation:} User sketches can be segmented via some clustering
algorithm and then information known to the third party about some members of the cluster can be generalized to the rest of the cluster. %For example, if a cluster contains users that have all responded to a particular type of campaign, then it is likely that the same campaign will work on the remaining users in the cluster.  The advertiser can thus directly translate the cluster into an actionable campaign strategy for that segment of users.
%Thus, segmentation can help control the advertiser's costs and reduce the experimentation needed when designing campaigns in order to personalize campaigns to users of different characteristics.
% Without segmentation, what is learned from one user only applies to that user. Segmentation enables generalization from a sample of users.
There is convincing evidence that segmentation of users into clusters is effective in some contexts \cite{bluekaiStudy,Millan,Mobasher,BT670}.

{\bf Nearest Neighbors:} Another application of perturbed
sketches is finding nearest neighbors. For example, finding users most similar to an already known one can be useful in the context of online dating, and product and movie recommendations.

\iffalse
For example, an advertiser who has a promotions budget that is not large enough to be offered to all users, may want to spend it on the users who are most likely to respond to the promotion. To do that, the advertiser can first learn who are the users who respond to good deals, and then use perturbed sketches to determine and target the  ``nearby" users. % sketches and design a campaign based on a good discount of their popular products.
Alternatively, an advertiser may select its `high end' users and seek other nearby users via the perturbed sketches. A campaign built around more upscale products could then be applied to the nearest neighbors. This ability to compute nearest neighbors offers advertisers a valuable and previously unavailable opportunity to evaluate how much a prospective user may be worth to them based on the value of the purchases (or other measures of ``worth'') made by users similar to the prospective one \cite{Evans}. %, which in turn, enables the advertisers to spend their advertising budget wisely.
One can imagine that in the future, search engines and ad networks will enable user-specific bidding, in which an advertiser, who knows a sketch of the characteristics of the user, is able to reflect the value of these characteristics to them through their bid. This could also be viewed as an intermediate solution between CPC and CPA auctions, offering the best of both \cite{Nazerzadeh08}.
\fi

\subsection{Limitations}
Although our algorithm offers a method for privacy-preserving sharing of user data with third parties in a way that enables user-user distance computations, there are other tasks for which the user data shared using our method would not be useful to third parties. We also discuss the limitations of the privacy protections we provide.

\subsubsection{Utility Limitations}
An important limitation of our work from the utility perspective is that the dimensions of the user sketches are impossible to interpret. As a consequence, the only way for a third party to select users satisfying a particular attribute is to project the vector corresponding to this attribute in the higher-dimensional space to the lower-dimensional space, and then perform the distance computation between user sketches and the obtained lower-dimensional attribute vector. However, as explained in \Section\ref{ss:comparison}, this computation would fall into the range of squared distance values for which both {\sc PrivateProjection} and {\sc RandomizedResponse} perform poorly. %Thus, our method does not enable third parties to identify users satisfying a particular attribute, unless they seek to identify users satisfying a fairly large list of attributes.

Furthermore, the proposed computation of user sketches weighs all attributes equally, which may not be desirable for third parties who want to prioritize similarity between users in some of the attributes over others. Computing multiple projections, each based on a different subset or weighing of the attributes would require use of additional privacy budget for each projection, as well as necessitate precluding the possibility of collusion among third parties.

Another limitation, which is a challenge for much of the privacy literature, is that our sketches provide a static snapshot of user data, and would require additional privacy budget in order to update them as the user information changes. The work of \cite{continuous} offers directions for possibly overcoming this challenge.

\iffalse
\subsubsection{Advertising Limitations}
While an advertiser can segment users and find nearest neighbors with
perturbed sketches, there is still quite a bit the advertiser cannot
do.  For example, the advertiser cannot see the queries that define a
cluster.  The actual search queries might aid the advertiser in
determining how to target a campaign.  The sequentiality of queries is
also lost in our transformation.

Furthermore, rather than computing Euclidean distances between user vectors, the advertiser might be interested in other relationships between them, e.g., dot product distance or cosine similarity. The dot product naturally arises if an advertiser wants to create a campaign consisting of search queries and determine which users exactly match this campaign. The first stab at (approximately) solving this problem would be to encode the campaign as a vector with $1$'s corresponding to indices of the queries desired and priors on the query probability in the other indices (which can be released with privacy \cite{DMNS06}), performing the projection on the campaign representation, and then operating in the Euclidean space according to our method. However, privacy-preserving sketches that do a better job of preserving dot product or cosine similarity is an important and promising direction for future work.


In addition, an advertiser cannot create a campaign of search queries
and match users that posed at least those search queries (or most of
them).  This definition of match is akin to the dot product distance
between a campaign vector and a user vector.  Note that in general,
preserving the Euclidean distance between vectors does not imply that
the dot product is preserved.  If an advertiser specifies a very short
campaign such as \{garmin\} $\wedge$ \{nuvi\} $\wedge$ \{gps\}, (which would correspond to a vector containing three $1$'s in positions corresponding to those queries, and containing $0.5$s elsewhere, encoding "indifference" for other features), a user
who poses the queries \{garmin\} and \{nuvi\} is almost as close to the campaign
in Euclidean distance ($\sqrt{\frac{d-3}{4}+1}$) as a user who poses just the query \{barbie\} ($\sqrt{4+\frac{d-4}{4}}$)---even though the latter user has nothing in common with the campaign.
Preserving the dot product is a very interesting and important
direction particularly for the information retrieval commmunity. We
leave this problem as a promising direction for future work. \comment{Should we leave this out: The
dimensionality reduction techniques presented in~\cite{moses1,moses2}
may be helpful.}

If both user and campaign vectors are normalized to the unit sphere,
then observe that the dot product is equivalent to the cosine of the
angle $\theta_{u,c}$ between user $u$ and campaign $c$, which is in
turn equivalent to the squared Euclidean distance between $u$ and $c$.
\[ \|u-c\|^2 = \|u\|^2 + \|c\|^2 - 2\|u\|\|c\| = 2 - 2 cos(\theta_{u,c}) \]
Further, observe that when $u$ and $c$ are close on the unit sphere,
then their squared Euclidean distances are also close, though an
approximation for one does not imply an approximation for the other.
\fi



\subsubsection{Privacy Limitations}
%Finally, we discuss limitations of our privacy protections.
While our work takes an important step forward, privacy
is more complex than ensuring that a third party cannot infer a particular attribute of a user. For example, if many of the attributes are correlated or representative of a higher-level user feature, then our techniques do not prevent a third party from inferring that.
In other words, our guarantees apply to a constant number of attributes, but not to a persistent trend that exists in the data.
Depending on the context, it may be more powerful to first categorize the attributes into
a coarser granularity prior to producing perturbed sketches. %, e.g., grouping all attributes corresponding to snow sports related interests such as skiing and snowboarding into a single attribute ``snow sports''.

Finally, as we explained in the Introduction, the goal of our work is to enable third parties to perform distance computations and clustering on users. Clearly, our work is not relevant for settings where such computations and privacy are fundamentally at odds, i.e., scenarios where the underlying data is so sensitive that even the ability to identify that two users are similar constitutes a privacy violation.


==> intro.tex <==
\section{Introduction}
In recent years, there has been an abundance of rich and fine-grained data about individuals in domains such as healthcare, finance, retail, web search and social networks. It is desirable for data collectors to enable third parties to perform complex data mining applications over such data. However, privacy is a natural obstacle that arises when sharing data about individuals with third parties, since the data about each individual may contain private and sensitive information.

We ask the following question: Is it possible to empower third parties with knowledge about users without compromising privacy of the users? Suppose that party A collects private information about its users, where each user's data is represented as a bit vector. We focus on the setting where a third party B has a proprietary data mining algorithm that requires estimating the distance between users, such as clustering or nearest neighbors. We ask if it is possible for party A to publish some information about each user so that B can estimate the distance between users without being able to infer any private bit of a user. Even in a scenario where the data mining algorithm is run by the data collector itself (that is, parties A and B are the same), privacy breaches are possible if the result of data mining is to be published \cite{FBattack10}. The reason is that complex algorithms that access private data can be susceptible to either unintended or adversarial attacks~\cite{CKN+11}. While one way to address this problem is to design a sophisticated algorithm that respects privacy (e.g., \cite{CMS08}), our approach can ensure that the data given as input to the algorithm itself does not compromise user privacy.

Although estimating distances between users in a privacy-preserving manner is a fundamental primitive in many data mining applications, the approaches known to date have certain short-comings. Approaches resorting to user id anonymization while keeping the data unchanged have been shown to be badly insufficient to preserve privacy \cite{nyt,netflixbreach}. A random projection based method to preserve distance between users was proposed in \cite{LiuKR06}, but later work demonstrated concrete attacks to breach privacy on this method \cite{Weakness1,Weakness2}. These approaches suffer due to lack of a rigorous privacy definition. On the other hand, approaches to data sharing such as the recently proposed provably private methods for search query and click data release \cite{Goetz,KKMN09} accomplish it at the price of giving up on all user-level information.


{\bf Contributions:}
We describe a simple, natural way to publish a sketch of a user that simultaneously preserves privacy and enables estimation of the distance between users.
%We represent a user by a vector over $d$ feature attributes.
The main idea is to project a $d$-dimensional vector representation of a user's feature attributes into a lower $k$-dimensional space by first applying a random Johnson-Lindenstrauss transform and then adding Gaussian noise $N(0,\sigma^2)$ to each bit of the resulting vector.  We prove that this perturbed lower-dimensional vector preserves differential privacy, i.e., an attacker who knows all but one attribute of a user cannot recover the value of that attribute from the published information with high confidence.
In terms of utility, we show how to recover the distance
between users from the perturbed sketches.  We show that the squared
Euclidean distance between pairs of users is preserved in expectation.
Further, with high probability, the distance between users is
preserved up to the usual Johnson-Lindenstrauss factors plus an
additive factor that depends on $k$ and the variance of the
noise $\sigma^2$.

We also compare our proposed solution to other candidate solutions.
For instance, we compare to the more straightforward solution of
directly adding noise to the user $\times$ user distance matrix.  We show that
in order to achieve the same privacy, the variance of the added noise
is higher for the more direct method.  Concretely,
we show that the projection-based method is better if the maximal
weight of a user vector is much smaller than the number of users.
Also, we analyze a
randomized response~\cite{warner} method for data sharing.
For a fixed value of the target dimension $k$, we show that for nearby points (those within squared distance $O(\sqrt k)$),
both algorithms are inaccurate.
Projection-based methods are better when pairs are medium distance apart,
i.e., between $\sqrt k$ and $\sqrt{dk} / \epsilon^2$.
Randomized response methods excel for pairs that are far apart.



\iffalse
To evaluate our algorithm, we experiment with one month of real search
logs as well as synthetic data. The goal of our experiments is to establish that pairwise
distances are preserved and the private sketches can be used for accurate clustering. Our experiments show that it is empirically possible to identify an optimum number of dimensions to project to, so that both privacy and distances are preserved.
Projecting to fewer dimensions yields poor results since dimension
reduction guarantees are not likely to hold, while projecting to many
dimensions implies adding noise to more dimensions, leading to
distorted distances.
\fi

While the problem of sharing data with third parties is more complex than producing sketches of user data that preserve distances between users, this work offers a privacy-preserving method to enable third parties to execute one of the core data-mining primitives. Since the goal of our work is to enable distance computations, understandably it does not apply in situations and applications where proximity to a particular user is itself sensitive information.






\iffalse
Over the last several years, many of the large online web services, such as Google, Yahoo! and Facebook, have accumulated a vast body of knowledge about individuals. Some of the services\footnote{Facebook Connect {\scriptsize \url{http://developers.facebook.com/blog/post/108/}}, Google Friend Connect {\scriptsize \url{http://www.google.com/friendconnect/}}} are actively looking for ways of sharing some of this user data with third parties, such as advertisers, other online services, application developers, or academic community. The goals of sharing are manyfold - from providing advertisers with better insights into users who are being exposed to their ads, to enabling other web services to provide a more personalized experience, to empowering application developers to create innovative products and technologies, and researchers to conduct studies at an unprecedented scale.

Privacy is a natural obstacle that arises when sharing data about individuals with \textit{third parties}, i.e., entities other than the one with whom the individual has interacted directly and entrusted with his information.
Privacy breaches are possible even in scenarios where third parties do not have direct access to such data but only to the output of running algorithms over the data. The reason is that complex algorithms that access private data can be susceptible to either unintended or adversarial attacks~\cite{CKN+11}. This problem can be addressed either by designing a sophisticated algorithm that respects privacy (e.g.,~\cite{CMS08}) or by ensuring that the data given as input to the algorithm itself does not compromise user privacy.

We ask the following question: Is it possible to empower third parties with knowledge about users without compromising their privacy? Rather than focusing on a specific knowledge domain or application, we aim to address the problem more broadly, studying an abstract data model for knowledge about users (each user is represented as a high-dimensional binary vector) and a general privacy model (each bit of the vector is potentially sensitive). We also ask whether we can generate privacy preserving version of the user data over which data mining algorithms can then be run.

The approaches known to date for such user data sharing have numerous short-comings. Those resorting to user id anonymization while keeping the data unchanged have been proven badly insufficient to preserve privacy \cite{nyt,netflixbreach}, others, such as the recently proposed provably private methods for search query and click data release \cite{KKMN09,Goetz} accomplish it at the price of giving up on all user-level information. We compare our proposed solution to randomized response~\cite{warner,ms}, a related method for data sharing, in \S~\ref{sec:randresponse}.

One of the key primitives useful for third party user data-mining applications is distance computation, i.e., the ability to measure distances between user feature representations and segment the users into clusters based on their distances. For example, in the context of search advertising, it has been shown~\cite{BT670} that customer segmentation can dramatically improve click through rates. \textbf{TODO: explain further and give references why preserving distances is helpful; other applications: OKCupid, Zimride carshare, Distance between people over movies they have rated together}

%Given that distance between users is the key to segmentation,
We thus rephrase the goal: is it possible to design a sketch of a user's data that simultaneously preserves user privacy and enables a third party to estimate the distance between users?
%The goal of the work is technical, to see whether the feat is possible without delving into nuances of concrete applications. Furthermore,
Since the goal of our work is to enable distance computations, understandably it does not apply in situations and applications where proximity to a particular user is itself sensitive information.


%Our method involves producing a noisy sketch of each user's data that can be published with their actual userid.  An evaluation of our technique on real search logs shows that even with privacy, distances can be approximately inferred.  While the problem of sharing data with third parties is more complex than producing sketches of user data that preserve distances between users, this work offers a privacy-preserving method to enable third parties to execute one of the core data-mining primitives.


{\bf Contributions:}
We propose a method to publish a sketch of a user
that simultaneously preserves privacy and enables estimation of the
distance between users.  %We represent a user by a vector over $d$ feature attributes.
The main idea is to project a $d$ dimensional vector representation of a user's feature attributes into a lower, random
$k$-dimensional space by first applying a Johnson-Lindenstrauss transform and then adding
Gaussian noise $N(0,\sigma^2)$ to each bit of the resulting vector.  We
prove that this perturbed lower-dimensional vector preserves
differential privacy, i.e., an attacker who knows all but one attribute of a user cannot recover the value of that attribute from the published information with high confidence.

In terms of utility, we give a method for recovering the distance
between users from the perturbed sketches.  We show that the squared
Euclidean distance between pairs of users is preserved in expectation.
Further, with high probability, the distance between users is
preserved up to the usual Johnson-Lindenstrauss factors plus an
additive factor that depends on $k$ and the variance of the
noise $\sigma^2$.


To evaluate our algorithm, we experiment with one month of real search
logs. \textbf{TODO: Update to reflect all experiments.} The goal of our experiments is to establish that pairwise
distances are preserved. Our experiments show that it is
empirically possible to identify an optimum number of dimensions to
project to, so that both privacy and distances are preserved.
Projecting to fewer dimensions yields poor results since dimension
reduction guarantees are not likely to hold, while projecting to many
dimensions implies adding noise to more dimensions, leading to
distorted distances.  Our experiments uncover an optimal number of
dimensions to project to so that distortion is minimized.

While the problem of sharing data with third parties is more complex than producing sketches of user data that preserve distances between users, this work offers a privacy-preserving method to enable third parties to execute one of the core data-mining primitives.

\fi


==> related.tex <==
\section{Related Work}
\iffalse
% Dropping since there is perhaps no need to motivate the need for data sharing across parties, and also to avoid drawing attention to online advertising
There is compelling evidence that third parties are clamoring for user data both online and offline. For example, Google analytics is used by 57\% of the 10,000 most popular websites\footnote{\scriptsize \url{http://trends.builtwith.com/analytics/Google-Analytics}}, more than 100,00 sites utilize the Facebook Connect API\footnote{\scriptsize \url{http://developers.facebook.com/blog/post/382}}, and the use of paid user data providers such as Rapleaf\footnote{\scriptsize \url{Rapleaf.com}} is rapidly growing. The desire to obtain additional information is motivated by belief that better knowledge of the potential user's characteristics and their similarity to others would enable third parties to create a more engaging, financially viable, social and personalized experience. On the other hand, users, advocacy groups, and legislators have
been voicing grave concerns about privacy risks posed
by their information re-sharing \textbf{cite{TODO}}.
\fi

Liu et al.~\cite{LiuKR06} introduce and motivate the problem of releasing data to third parties with a goal that the original sensitive information cannot be inferred while preserving analytic properties of the data, such as inner product and Euclidean distance computations. Their approach is based on random projection to a lower-dimensional subspace using a projection matrix drawn from a distribution unknown to the adversary. The key distinction from our work is that they do not utilize an operational definition for what it means to protect the privacy of the data, and therefore, as they point out, there are scenarios in which an adversary can find approximations to original data (e.g., if the data is restricted to Boolean domain or adversary possesses certain background knowledge). Follow-up works~\cite{Weakness1,Weakness2} propose concrete attacks and demonstrate the vulnerabilities of the approach. Our use of differential privacy and addition of properly calibrated random noise after the projection enables us to provide a rigorous privacy guarantee, as well as gain insight into the change in utility depending on projected dimension used. Mukherjee et al.~\cite{Mukh} propose enabling distance-based mining algorithms over private data using Fourier-related transforms, but their approach has the same drawbacks as Liu et al.~\cite{LiuKR06}.

\iffalse
% Not directly related
There is extensive work on enabling privacy-preserving data mining for various applications (e.g., for  association rule mining \cite{EvfimievskiSAG02, Bhaskar10}). We focus the rest of the related work discussion on techniques whose explicit goal is enabling private distance computations or clustering.
\fi

We discussed randomized response in \Section\ref{sec:randresponse} and compared its performance with our method in \Section\ref{ss:comparison}. In terms of privacy, randomized response offers a slightly better privacy
guarantee. However, from a utility perspective, randomized response
does not preserve ``small'' distances as effectively as the present
work.  Concretely, for users that are less than $\sqrt{dk}$ distance
apart, our method provides stronger guarantee than randomized response.
Since third parties are likely interested in preserving
small distances, we believe that our approach is more suitable for
typical data mining applications.

\iffalse
Regarding output perturbation, one solution
is for a search engine to not publish any data and only allow
black-box queries to the search data where answers to queries are
perturbed~\cite{DMNS06,pinq}.  Prior work shows how cluster centers
can be approximately computed~\cite{bdmn}, but the goal differs in
that we seek to let advertisers know which users belong to which
cluster.  Our work strikes a balance between input and output
perturbation methods.
\fi

From a differential privacy perspective,
alternative solutions could be used to attack our problem.  For
example, Blum et al.~\cite{bdmn} give a method of running $k$-Means on
a private data set maintained by a trusted administrator.  Their goal is to produce $k$ cluster centers that are not too far from the $k$ cluster centers that $k$-Means would
produce if the algorithm had access to the private data.  Our goal differs in that we seek to publish data (or enable its utilization) along with the userIDs and enable identification of users who belong to the same cluster.  Also, our noisy sketches can also be used for other distance-based computations such as nearest neighbors. Finally, another possible direction is not to publish any data and only allow black-box queries to the first-party data provider, where the answers to such queries are perturbed~\cite{DMNS06,pinq}. This approach may place considerable burden on the first-party data provider, and consumes privacy budget with each query posed.


\iffalse
\section{Related Work}
%\subsubsection{The power of behavioral targeting}
In the last several years, behavioral targeting, a technique that uses the user's online activity in order to
% uses information collected about users based on their online activities in order to categorize their interests, and then use the categorization to
target personalized ads to them, has been gaining prominence. The online activities can include the information the users posts about themselves on a social networking site, as well as their web browsing behavior, their search queries, and purchase history.

It has been shown that users with similar search and browsing behavior have similar interests and therefore higher probability to click the same ad, and therefore, behavioral targeting can improve the relevance of ads displayed to users and yield astounding improvements in click-through rates, of up to 670\% \cite{BT670, Clarke}. The leading advertising brokers such as Google\footnote{\url{http://www.google.com/privacy_ads.html}} and Yahoo\footnote{\url{http://info.yahoo.com/privacy/us/yahoo/relevantads.html}}%, LinkedIn\footnote{\url{https://www.linkedin.com/secure/settings?lan=&goback=.aas}}  are rapidly adopting it
have recently adopted behavioral targeting, with the hope that the technique improves ad relevance, and hence, both the user experience and monetization potential.

Furthermore, today's online advertisers actively seek to go beyond the click-through rate in understanding the performance of their advertising campaigns, as well as the user behavior that leads to conversion \cite{Muthu10}. This is motivated by belief \cite{Evans} that better knowledge of the potential customer's characteristics, search and browsing history, would enable the advertiser to create more catchy campaigns, landing pages, and personalized offers. For example, a high-end shoe retailer might be interested in knowing whether the user has been recently searching for "Manolo Blahnik" or "cheap shoes", and whether they regularly visit celebrity websites or discount store websites, in order to better evaluate the value to them of displaying the ad to that user, or which types of shoes to highlight once the user visits their page. The evidence that the advertisers are scrambling to obtain as much information as they can about the users ranges from the popularity of various Analytics solutions, such as Google Analytics (used by 57\% of the 10,000 most popular websites\footnote{\url{http://trends.builtwith.com/analytics/Google-Analytics}}), to participation in Advertising Exchanges (e.g., Right Media, DoubleClick), engagement with audience targeting marketplaces such as BlueKai\footnote{\url{bluekai.com}} and Rapleaf\footnote{\url{Rapleaf.com}}, and practice of embedding the search terms customers used to find a retailer's coupon into the coupon bar code itself \cite{Coupons}.


%Users with similar search and browsing behavior have similar interests and therefore higher probability to click the same ad \cite{BT670}. Segmentation of users into small groups for ad delivery. USers who click the same ad can be 90 times more similar than users who clicked different ads. User search queries can perform several times better than user browsing behaviors.
%
%\cite{Muthu08} poses ad effectiveness estimation for different target groups as well as inferring profiles as important open problems for ad auctions. Advertisers seek to go beyond the click-through rate in understanding the performance of their advertising campaigns as well as the user behavior that leads to conversion. \cite{Muthu10} takes an approach of introducing a graph-based framework for reporting the various paths the user took before conversion.
%
%Evidence of advertisers trying to obtain user information are the ad exchanges, Right Media, DoubleClick, BlueKai.
%
%For example, an advertiser of high-end shoes such as Manolo Blahnik might value impressions served to fashion-obsessed wealthy women much more than impressions to sporty teenagers. If the advertiser is able to receive a sketch of a user's interests, and has a history of sketches of other users and their conversions, then they would be able to
%\url{http://www.mikeonads.com/2007/07/26/selling-behavioral-data-in-a-multi-platform-ad-industry/}

%The advertisers are hungry to improve performance of their campaigns.
%\cite{Evans} Data on what people have search online could determine whether a particular individual exhibits characteristics that makes them a good target for the ad, and whether it is worth paying a premium.

%Behavioral targeting is a rapidly developing field and techniques for it are in the discovery process. One approach to behavioral targeting is to segment visitors of a site into groups, and then use a distinct approach to each group. In order to perform this segmentation, the ad brokers utilize user history, profile information, toolbar logs, etc. to build up profiles of users.
%How it's currently done, coupons, advertisers; currently on a query basis but there's a gradual shift to behavioral targeting.

%\subsubsection{Advertising leaks private data}
On the other hand, the online users, advocacy groups, and legislators have been voicing grave concerns \cite{Hoofnagle} about privacy risks posed by behavioral targeting, especially in the context of the data collected by ad brokers being shared with outside entities, e.g., advertisers. %For example, after a recent Wall Street Journal article detailing the practice of such data collection by RapLeaf, more than XXX users chose to opt out in one day.
%The danger that behavioral advertising poses to user privacy has been a topic of hot debate in the industry, academia, and government.
The most prominent example of their concerns is the uproar, including a class action law suit\footnote{\url{http://searchengineland.com/class-action-suit-targets-google-seeks-elmination-of-search-query-sharing-53895}, \url{http://www.scribd.com/doc/40116745/2010-10-25-FINAL-Complaint}}, surrounding "referrers", %While many of the users understand that Most of the concerns discussed so far have focused on "referrer" data, the practice
the practice in which the user id or search query is passed along to the advertiser by the ad broker when the user clicks on the ad. In the social network context, the danger of the practice is imminently clear - through a referrer containing the unique user id, the advertiser can tie the click to a particular user's identity \cite{Wills, Edelman, Steel}.
%\cite{FBattack10, Guha}.
%Leaks through referrer urls sent \cite{Wills, Edelman, Steel} who have shown that clicking on a Facebook ad, in some cases, revealed to the advertiser the user ID of the person clicking, due to Facebook's failure to properly anonymize the HTTP Referer header. Their work has resulted in much publicity and Facebook has since fixed this vulnerability \cite{FBreferer}.
%Leaks through advertising \cite{FBattack10, Guha, Helft}
In the search engine context, the danger comes from profile information containing distinctly identifying queries, e.g., so called \textit{vanity searches} \cite{Vanity}, which, when combined together with other searches, such as "HIV" and "rape" can lead to a possibility of private information leakage \cite{SoghoianVanity}.


%\subsubsection{Potential fixes}
The ability to perform behavioral targeting and communicate user information in a way that empowers advertisers to improve their campaigns but without violating user privacy is becoming one of the most important questions facing the industry.

On the technical solution side, the Adnostic~\cite{Adnostic} and Privad~\cite{Guha09servingads} projects embody systems that perform ad selection and targeting on the user's side through a browser extension, and use cryptographic techniques for accounting. These proposals are likely to face barriers in adoption, as they require a shift in the paradigm of online advertising, where the ad brokers relinquish their control of the way matching is performed and the matching itself relies on a weaker client-side model of the user than the rich models the ad brokers have built up. Furthermore, these proposals do little to empower the advertisers in learning more about their users in order to improve their ability to provide personalized experience.

%The choice of which ads to show and serving of the ads is performed locally on a users computer \cite{Guha09servingads}. Both unlikely to gain widespread adoption in the near term by major ad brokers such as Facebook and Google, due to their limitations in their power, the system the marketers have come to expect, etc. Does not deal with confidentiality for advertisers.

On the policy side, self-regulation and consumer education about behavioral advertising has been heavily encouraged and embraced by many industry players, most notably, through the Network Advertising Initiative \footnote{\url{http://www.networkadvertising.org/}}. The initiative provides users with a central place to opt-out of cookies placed by the NAI's members but does not protect users from their private data leakage through referrers. Furthermore, a complete opt-out, while protecting some privacy, also does users a disservice by removing the ability of the ad network to tailor the ads to that user's specific interests. %behavioral advertising, a solution that but the solution of , and to give users more explanations and control, which contributes to an illusion of privacy.

%On the usability side, the "Power-Eye" technology \cite{PowerEye, Better}, which allows consumers to mouse over the ad to get a view of the data that was used to target the ad, offers some hope in providing the user with the understanding of the information they might be revealing when clicking on a particular ad. However, the hassle and understanding of privacy issues required to evaluate the breadth of the targeting and the risk that it poses is beyond the ability of a typical consumer, so the technology may, in fact, be providing an illusion of privacy and control.
%and thus, the best solution from the perspective of protecting one's privacy is to avoid clicking any of the ads.

%FTC to recommend self-regulation not new laws for behavioral targeting
%\url{http://www.mediapost.com/publications/?fa=Articles.showArticle&art_aid=137984}

%Some solutions based on network anonymity have also been proposed. \\
%Tor, TrackMeNot

%Some ad-hoc solutions \\
Finally, a combination of ad-hoc approaches, such as providing very coarse characteristic information \footnote{\url{https://www.google.com/adplanner/}} or only the most recent user query through referrer to advertisers, is what is being used at the moment, which falls far short of the detailed information about the users that advertisers aspire for.

The best solutions for empowering advertisers while preserving user privacy is still up in the air, and in this work we propose a first step towards design of behavioral targeting systems capable of sharing segmentation and distance between users information with advertisers in a provably private manner. Our technique falls inbetween input and output perturbation approaches to preserving privacy. \comment{TODO: elaborate on other privacy techniques}.

\subsubsection{Attacks}
\cite{GoogleJob}
\cite{CastellucciaCP10}

\cite{nyt, Tomkins07}

\cite{Vanity, SoghoianVanity}

\cite{Guha} and demonstrated \cite{FBattack10}

33 bits \cite{Panopticlick, Eckersley, 33bits}

%
%\subsubsection{Why need rigorous privacy proofs}
%In response to the most recent reports \cite{Steel} on leakage of Facebook data to the advertisers, Harry Lewis\cite{Lewis} poses a question of "Why does this keep happening?" and conjectures that it's "Surely not by design on Facebook's part". We believe that the fundamental problem of designing systems or releasing data based on heuristic notions of privacy is that adversaries can always come up with more sophisticated and unanticipated ways to breach the heuristic protections. We therefore believe that for any system in which protection of user privacy is important, it is crucial to design the system with provable privacy guarantees.
%
%Furthermore, an advertising attack is a bigger threat than a spam attack. Spammers need to be active, creating accounts, commenting, actively exploring people, etc. For an advertising attack, one just needs "sleeper" accounts that become active once in a while, a behavior that is much harder to catch.



\fi 
